Abstract Meaning Representation for Hospital Discharge Summarization

The Achilles heel of Large Language Models (LLMs) is hallucination, which has drastic consequences for the clinical domain. This is particularly important with regards to automatically generating discharge summaries (a lengthy medical document that summarizes a hospital in-patient visit). Automatically generating these summaries would free physicians to care for patients and reduce documentation burden. The goal of this work is to discover new methods that combine language-based graphs and deep learning models to address provenance of content and trustworthiness in automatic summarization. Our method shows impressive reliability results on the publicly available Medical Information Mart for Intensive III (MIMIC-III) corpus and clinical notes written by physicians at Anonymous Hospital. rovide our method, generated discharge ary output examples, source code and trained models.

==> makefile <==
# Paul Landes - 6/20/2018
# export version makefile
# https://github.com/plandes/zenbuild
#
# To build you need:
#   - Latex2e
#   - pdflatex
#   - either bibtex or biber if `zenbiber` is present
#   - GNU make


## setup

# binaries
TEX_LATEX_CMD =	pdflatex
BIBTEX=		bibtex
BIBER=		biber
BIB_FILE=	$(wildcard *.bib)

# files
TEX=		ClinicalALignmentSUMmarization
TEX_LATEX_FILE=	$(TEX).tex
TEX_PDF_FILE=	$(TEX).pdf
TEX_FINAL_RUNS =2


## targets

# default target
all:		pdf

# build information
.PHONY:		info
info:
		@echo "name: $(TEX)"
		@echo "tex: $(TEX_LATEX_FILE)"
		@echo "pdf: $(TEX_PDF_FILE)"
		@echo "bib-file: $(BIB_FILE)"

# build the PDF file
.PHONY:		pdf
pdf:		$(TEX_PDF_FILE)

$(TEX_PDF_FILE):	$(TEX_LATEX_FILE)
		$(TEX_LATEX_CMD) $(TEX).tex
		if [ -f "$(BIB_FILE)" ] ; then \
			if [ -f zenbiber ] ; then \
				$(BIBER) $(TEX) ; \
			else \
				$(BIBTEX) $(TEX) ; \
			fi \
		fi
		for i in `seq $(TEX_FINAL_RUNS)` ; do \
			$(TEX_LATEX_CMD) $(TEX).tex ; \
		done

# clean a used build
clean:
		rm -f *.pdf *.out *.aux *.log *.bbl *.bcf *.blg \
			*.upa *.upb *.xml

